Assessing Evaluation Metrics for Neural Test Oracle Generation

In this work, we revisit existing oracle generation studies plus ChatGPT to empirically investigate the current standing of their performance in both NLG-based and test adequacy metrics. Specifically, we train and run four state-of-the-art test oracle generation models on five NLG-based and two test adequacy metrics for our analysis. We apply two different correlation analyses between these two different sets of metrics. Surprisingly, we found no significant correlation between the NLG-based metrics and test adequacy metrics. For instance, oracles generated from ChatGPT on the project activemq-artemis had the highest performance on all the NLG-based metrics among the studied NOGs, however, it had the most number of projects with a decrease in test adequacy metrics compared to all the studied NOGs. We further conduct a qualitative analysis to explore the reasons behind our observations, we found that oracles with high NLG-based metrics but low test adequacy metrics tend to have complex or multiple chained method invocations within the oracle's parameters, making it hard for the model to generate completely, affecting the test adequacy metrics. On the other hand, oracles with low NLG-based metrics but high test adequacy metrics tend to have to call different assertion types or a different method that functions similarly to the ones in the ground truth. Overall, this work complements prior studies on test oracle generation with an extensive performance evaluation with both NLG and test adequacy metrics and provides guidelines for better assessment of deep learning applications in software test generation in the future.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> figures/approach.tex <==
\begin{figure*}[ht!]
    \centering
     \resizebox{0.8\textwidth}{!}{{\includegraphics{figures/approach.pdf}}}    
     \caption{The overview of our experiment approach.}
     % \song{"from test set" is inappropriate here, you can remove it}
    \label{fig:approach}
\end{figure*}



==> figures/rq3_linechart.tex <==
\pgfplotsset{compat=1.14}

%enter the data sets as follows.


\begin{figure}[h!]
\begin{tikzpicture}
\begin{axis}[
    axis lines=bottom,
    ymin=-0.02,
    % x label style={at={(current axis.right of origin)},anchor=north, below=1mm},
    % title={\textit{\textbf{BLEU, LC, and MS}}},
    xlabel=BLEU,
    ylabel=Metric scores,
    % xticklabel style = {rotate=30,anchor=east},
    enlargelimits = false,
    % xticklabels from table={thu2.dat}{Time},xtick=data
    legend style={at={(0.5, 1.02)},anchor=south}
]
\addplot[orange,dotted,mark=*] table [y=BLEU,x=X]{thu2.dat};
\addlegendentry{BLEU}
\addplot[green,dotted,mark=*] table [y= LC,x=X]{thu2.dat};
\addlegendentry{Line coverage}]
\addplot[blue,dotted,mark=*] table [y=MS,x=X]{thu2.dat};
\addlegendentry{Mutation score}
\end{axis}
\end{tikzpicture}
\caption{Comparison between BLEU, line coverage, and mutation score.}
% \song{the yellow line is METEOR or BLEU?}
% \jiho{it is bleu score, I changed it accordingly}
\end{figure}

==> sec/motivation.tex <==
\section{Motivation}
\label{sec:motivation}

% \song{revise this section by giving examples with higher NLG metric values while low adequacy}

% The common data used in neural oracle generation is from \emph{ATLAS} \cite{watson2020learning}.

% There are three main studies regards to neural oracle generation, i.e. \emph{ATLAS}, \emph{IR}, \emph{TOGA}.
% The followings are the NOG studies that have been published in major software engineering venues and arXiv within the three years.
%Watson et al. \cite{watson2020learning} proposed \emph{ATLAS} which is the first study to generate assert statements for Java unit tests using deep neural networks. They treat oracle generation as neural machine translation. By feeding the test prefix and the focal method, the model translates by generating its line of oracle.
%White and Krinke \cite{white2020reassert} proposed \emph{ReAssert} that targets specific projects to generate oracle statements from focal methods only, i.e. without test prefixes.
%Mastropaolo et al. \cite{mastropaolo2021studying, mastropaolo2022using} did an empirical study on T5 (\underline{T}ext-\underline{T}o-\underline{T}ext \underline{T}ransfer \underline{T}ransformer) models on its effect on code related tasks. They assessed different software engineering-related tasks, i.e. automatic program repair, code mutant injection, assertion generation, and code summarization.
%Yu and Lout et al. \cite{yu2022automated} proposed \emph{IR} which they integrate an information retrieval method on \emph{ATLAS} to improve the effectiveness of its generation ability. They have added a new dataset that includes the dropped instances with unknown vocabulary from \emph{ATLAS} in their filtering step.
% Their new dataset consists 265,420 of test-oracle pairs.
%Dinella et al. \cite{dinella2022toga} proposed \emph{TOGA} which is a test oracle generator that generates both exceptional oracles and assertion oracles. First, the tool decides if the test prefix should handle an exception. If it does not, it further generates candidate assertion lines. Within the generated candidate assertions, it will rank them with probability and suggest the first-rank assertion. They adopted \emph{Methods2Test} \cite{tufano2022methods2test} dataset, which is a dataset for whole unit test case generation when a focal method is given to evaluate their exceptional oracle generation.
%Tufano et al. \cite{tufano2022generating} propose a transformer-based method to generate assert oracles for unit test cases, which leverages transfer learning from English and source code corpora. They show that their method outperforms a previous RNN-based method and can improve test coverage by augmenting EvoSuite test cases. 

As discussed in Section \ref{sec:back-ass-gen}, former studies mainly used NLG-based metrics such as BLEU, CodeBLEU, ROUGE-L, METEOR,
and accuracy to evaluate the generation performance of the models. 
%We also found studies that additionally evaluated the dynamic or the test adequacy attributes of the generated oracle.
%The dynamic evaluations these studies performed include simple methods such as counting the passing and compiling test methods (ReAssert \cite{white2020reassert}) and more complex evaluations such as false positive rate (FPR) of the bug detection ability (TOGA \cite{dinella2022toga}) and test coverage (Tufano et al. \cite{tufano2022generating}). 
%However, the complexity and the scale of the execution evaluation have limitations, \emph{ReAssert} having limitation in complexity, \emph{TOGA} and Tufano et al. having limitations in scale (120 bugs and 18 test methods respectively).
%We can see that the current field of neural assertion generation heavily relies on NLG-based metrics and a limited amount of them explore its effectiveness concerning the dynamic or the test adequacy metrics.
While, we find that the NLG-based metric cannot fully reflect the test adequacy. 
Consider the following example in Listing \ref{lst:motive}, which shows an input and output example of an oracle generated by \add{xxx model}.  
When the model receives an aggregation of the test prefix and the focal method, it generates an appropriate oracle that will go into the \emph{"<AssertPlaceHolder>"}.
As we can see, the generated oracle and the ground truth oracle function the same (i.e., check whether `in' is null or not) with different types of assertion, hence the same test adequacy with the ground truth.
However, the corresponding BLEU score for the generated oracle in a very low score of 3.66.
This calls for a more thorough investigation of the use of NLG-based metrics and test adequacy metrics in evaluating oracle generation tasks and their correlation. 
\input{figures/motive_ex}
% This calls for attention to further assess the NOG models' performance as these metrics could have limitations in conveying the quality of oracles as mentioned in previous studies \cite{reiter2018structured, mathur2020tangled, leclair2019recommendations, stapleton2020human, roy2021reassessing}.


%For a more comprehensive empirical study, we added three more NLG-based metrics, i.e. CodeBLEU, METEOR, and ROUGE-L.
%We also want to assess the quality of the oracles at the execution level using test adequacy metrics.
%These metrics are used in automatic test case generation to assess the quality and the strength of the generated test case.
%After we get both metrics, we investigate the correlation of these two metrics together with quantitative manual analysis for more discussion.
% \jiho{add example code of high static but low dynamic scores}
% We want to further investigate the cause of great improvement in this field especially when using the dataset \emph{ATLAS}.
% We check for any possible information leakage across the different splits, i.e. across training, validation, and the test set as this is spotted as a problem in training source code \cite{allamanis2019adverse, russell2018automated, kang2022detecting}.
% Second, we want to see if there is data duplication in the dataset as this can cause inflation in the performance evaluation metrics \cite{kang2022detecting, allamanis2019adverse}.

% \emph{ATLAS} \cite{watson2020learning}
% is a parallel dataset consisting of a test prefix and the focal method as input and the oracle line as output.
% The dataset focuses on Java projects that use the JUnit testing framework.

% \subsection{Information Leakage}
% To avoid any information leakage introduced to evaluated splits from the training split, we first need to group the instances by their projects.
% After newly processing the dataset, we investigate how the existing oracle generation models perform on them.
% How we processed the dataset is explained in Section \ref{sec:dataset}

% \subsection{Data duplication}

==> tables/rq3_atlas.tex <==
\begin{table}[t!]
\caption{The result of correlation analysis for \emph{ATLAS}. The bold shows the P-value that is less than 0.05.}
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|lll|lll|}
\cline{2-7}
\textbf{} & \multicolumn{3}{c|}{\textbf{Spearman's}} & \multicolumn{3}{c|}{\textbf{Kendall's}} \\ \hline
\multicolumn{1}{|l|}{\textbf{Metrics}} & \multicolumn{1}{l|}{\textbf{$\rho$}} & \multicolumn{1}{l|}{\textbf{Z score}} & \textbf{P-value} & \multicolumn{1}{l|}{\textbf{$\tau$}} & \multicolumn{1}{l|}{\textbf{Z score}} & \textbf{P-value} \\ \hline
\multicolumn{1}{|l|}{LC vs BLEU} & \multicolumn{1}{l|}{0.3736} & \multicolumn{1}{l|}{1.2060} & 0.1139 & \multicolumn{1}{l|}{0.2051} & \multicolumn{1}{l|}{0.9798} & 0.1636 \\ \hline
\multicolumn{1}{|l|}{LC vs EM} & \multicolumn{1}{l|}{0.2228} & \multicolumn{1}{l|}{0.6961} & 0.2432 & \multicolumn{1}{l|}{0.1936} & \multicolumn{1}{l|}{0.9232} & 0.1780 \\ \hline
\multicolumn{1}{|l|}{LC vs CB} & \multicolumn{1}{l|}{0.1813} & \multicolumn{1}{l|}{0.5631} & 0.2867 & \multicolumn{1}{l|}{0.1538} & \multicolumn{1}{l|}{0.7348} & 0.2312 \\ \hline
\multicolumn{1}{|l|}{LC vs RL} & \multicolumn{1}{l|}{0.5275} & \multicolumn{1}{l|}{1.8018} & \textbf{0.0358} & \multicolumn{1}{l|}{0.3846} & \multicolumn{1}{l|}{1.8371} & 0.0331 \\ \hline
\multicolumn{1}{|l|}{LC vs MT} & \multicolumn{1}{l|}{0.3956} & \multicolumn{1}{l|}{1.2852} & 0.0994 & \multicolumn{1}{l|}{0.3077} & \multicolumn{1}{l|}{1.4697} & 0.0708 \\ \hline
\multicolumn{1}{|l|}{MS vs BLEU} & \multicolumn{1}{l|}{0.4560} & \multicolumn{1}{l|}{1.5121} & 0.0653 & \multicolumn{1}{l|}{0.3077} & \multicolumn{1}{l|}{1.4697} & 0.0708 \\ \hline
\multicolumn{1}{|l|}{MS vs EM} & \multicolumn{1}{l|}{0.3164} & \multicolumn{1}{l|}{1.0062} & 0.1572 & \multicolumn{1}{l|}{0.2452} & \multicolumn{1}{l|}{1.1694} & 0.1211 \\ \hline
\multicolumn{1}{|l|}{MS vs CB} & \multicolumn{1}{l|}{0.2582} & \multicolumn{1}{l|}{0.8116} & 0.2085 & \multicolumn{1}{l|}{0.2051} & \multicolumn{1}{l|}{0.9798} & 0.1636 \\ \hline
\multicolumn{1}{|l|}{MS vs RL} & \multicolumn{1}{l|}{0.6264} & \multicolumn{1}{l|}{2.2588} & \textbf{0.0119} & \multicolumn{1}{l|}{0.4359} & \multicolumn{1}{l|}{2.0821} & 0.0187 \\ \hline
\multicolumn{1}{|l|}{MS vs MT} & \multicolumn{1}{l|}{0.5110} & \multicolumn{1}{l|}{1.7325} & \textbf{0.0416} & \multicolumn{1}{l|}{0.3590} & \multicolumn{1}{l|}{1.7146} & 0.0432 \\ \hline
\end{tabular}}
\label{tab:rq3_atlas}
\end{table}

==> tables/rq3_chatgpt.tex <==
\begin{table}[t!]
\caption{The result of correlation analysis for \emph{ChatGPT}.}
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|lll|lll|}
\cline{2-7}
& \multicolumn{3}{c|}{\textbf{Spearman's}} & \multicolumn{3}{c|}{\textbf{Kendall's}} \\ \hline
\multicolumn{1}{|l|}{\textbf{Metrics}} & \multicolumn{1}{l|}{\textbf{rho}} & \multicolumn{1}{l|}{\textbf{Z score}} & \textbf{P-value} & \multicolumn{1}{l|}{\textbf{tau}} & \multicolumn{1}{l|}{\textbf{Z score}} & \textbf{P-value} \\ \hline
\multicolumn{1}{|l|}{LC vs BLEU} & \multicolumn{1}{l|}{0.0549} & \multicolumn{1}{l|}{0.1689} & 0.4329 & \multicolumn{1}{l|}{0.0513} & \multicolumn{1}{l|}{0.2449} & 0.4032 \\ \hline
\multicolumn{1}{|l|}{LC vs EM} & \multicolumn{1}{l|}{0.3022} & \multicolumn{1}{l|}{0.9581} & 0.1690 & \multicolumn{1}{l|}{0.2308} & \multicolumn{1}{l|}{1.1023} & 0.1352 \\ \hline
\multicolumn{1}{|l|}{LC vs CB} & \multicolumn{1}{l|}{0.2779} & \multicolumn{1}{l|}{0.8765} & 0.1904 & \multicolumn{1}{l|}{0.1677} & \multicolumn{1}{l|}{0.8078} & 0.2096 \\ \hline
\multicolumn{1}{|l|}{LC vs RL} & \multicolumn{1}{l|}{0.3297} & \multicolumn{1}{l|}{1.0519} & 0.1464 & \multicolumn{1}{l|}{0.2564} & \multicolumn{1}{l|}{1.2247} & 0.1103 \\ \hline
\multicolumn{1}{|l|}{LC vs MT} & \multicolumn{1}{l|}{0.2912} & \multicolumn{1}{l|}{0.9211} & 0.1785 & \multicolumn{1}{l|}{0.2308} & \multicolumn{1}{l|}{1.1023} & 0.1352 \\ \hline
\multicolumn{1}{|l|}{MS vs BLEU} & \multicolumn{1}{l|}{0.1374} & \multicolumn{1}{l|}{0.4246} & 0.3356 & \multicolumn{1}{l|}{0.1282} & \multicolumn{1}{l|}{0.6124} & 0.2701 \\ \hline
\multicolumn{1}{|l|}{MS vs EM} & \multicolumn{1}{l|}{0.4341} & \multicolumn{1}{l|}{1.4279} & 0.0767 & \multicolumn{1}{l|}{0.3590} & \multicolumn{1}{l|}{1.7146} & 0.0432 \\ \hline
\multicolumn{1}{|l|}{MS vs CB} & \multicolumn{1}{l|}{0.2063} & \multicolumn{1}{l|}{0.6430} & 0.2601 & \multicolumn{1}{l|}{0.1419} & \multicolumn{1}{l|}{0.6835} & 0.2471 \\ \hline
\multicolumn{1}{|l|}{MS vs RL} & \multicolumn{1}{l|}{0.4176} & \multicolumn{1}{l|}{1.3661} & 0.0860 & \multicolumn{1}{l|}{0.2821} & \multicolumn{1}{l|}{1.3472} & 0.0890 \\ \hline
\multicolumn{1}{|l|}{MS vs MT} & \multicolumn{1}{l|}{0.4505} & \multicolumn{1}{l|}{1.4909} & 0.0680 & \multicolumn{1}{l|}{0.3077} & \multicolumn{1}{l|}{1.4697} & 0.0708 \\ \hline
\end{tabular}}
\label{tab:rq3_chatgpt}
\end{table}

==> tables/rq3_ir.tex <==
\begin{table}[t!]
\caption{The result of correlation analysis for \emph{IR}.}
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|lll|lll|}
\cline{2-7}
\textbf{} & \multicolumn{3}{c|}{\textbf{Spearman's}} & \multicolumn{3}{c|}{\textbf{Kendall's}} \\ \hline
\multicolumn{1}{|l|}{\textbf{Metrics}} & \multicolumn{1}{l|}{\textbf{$\rho$}} & \multicolumn{1}{l|}{\textbf{Z score}} & \textbf{P-value} & \multicolumn{1}{l|}{\textbf{$\tau$}} & \multicolumn{1}{l|}{\textbf{Z score}} & \textbf{P-value} \\ \hline
\multicolumn{1}{|l|}{LC vs BLEU} & \multicolumn{1}{l|}{0.2063} & \multicolumn{1}{l|}{0.6430} & 0.2601 & \multicolumn{1}{l|}{0.1161} & \multicolumn{1}{l|}{0.5550} & 0.2895 \\ \hline
\multicolumn{1}{|l|}{LC vs EM} & \multicolumn{1}{l|}{0.1350} & \multicolumn{1}{l|}{0.4172} & 0.3383 & \multicolumn{1}{l|}{0.0520} & \multicolumn{1}{l|}{0.2479} & 0.4021 \\ \hline
\multicolumn{1}{|l|}{LC vs CB} & \multicolumn{1}{l|}{0.1458} & \multicolumn{1}{l|}{0.4511} & 0.3260 & \multicolumn{1}{l|}{0.1161} & \multicolumn{1}{l|}{0.5550} & 0.2895 \\ \hline
\multicolumn{1}{|l|}{LC vs RL} & \multicolumn{1}{l|}{0.4044} & \multicolumn{1}{l|}{1.3174} & 0.0939 & \multicolumn{1}{l|}{0.3484} & \multicolumn{1}{l|}{1.6649} & 0.0480 \\ \hline
\multicolumn{1}{|l|}{LC vs MT} & \multicolumn{1}{l|}{0.1868} & \multicolumn{1}{l|}{0.5806} & 0.2808 & \multicolumn{1}{l|}{0.1538} & \multicolumn{1}{l|}{0.7348} & 0.2312 \\ \hline
\multicolumn{1}{|l|}{MS vs BLEU} & \multicolumn{1}{l|}{0.1183} & \multicolumn{1}{l|}{0.3650} & 0.3575 & \multicolumn{1}{l|}{0.0645} & \multicolumn{1}{l|}{0.3083} & 0.3789 \\ \hline
\multicolumn{1}{|l|}{MS vs EM} & \multicolumn{1}{l|}{0.2039} & \multicolumn{1}{l|}{0.6350} & 0.2627 & \multicolumn{1}{l|}{0.1559} & \multicolumn{1}{l|}{0.7437} & 0.2285 \\ \hline
\multicolumn{1}{|l|}{MS vs CB} & \multicolumn{1}{l|}{0.1843} & \multicolumn{1}{l|}{0.5727} & 0.2834 & \multicolumn{1}{l|}{0.1161} & \multicolumn{1}{l|}{0.5550} & 0.2895 \\ \hline
\multicolumn{1}{|l|}{MS vs RL} & \multicolumn{1}{l|}{0.2944} & \multicolumn{1}{l|}{0.9317} & 0.1758 & \multicolumn{1}{l|}{0.2452} & \multicolumn{1}{l|}{1.1716} & 0.1207 \\ \hline
\multicolumn{1}{|l|}{MS vs MT} & \multicolumn{1}{l|}{0.1319} & \multicolumn{1}{l|}{0.4074} & 0.3419 & \multicolumn{1}{l|}{0.1026} & \multicolumn{1}{l|}{0.4899} & 0.3121 \\ \hline
\end{tabular}}
\label{tab:rq3_ir}
\end{table}

==> tables/rq3_toga.tex <==
\begin{table}[t!]
\caption{The result of correlation analysis for \emph{TOGA}.}
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|lll|lll|}
\cline{2-7}
\textbf{} & \multicolumn{3}{c|}{\textbf{Spearman's}} & \multicolumn{3}{c|}{\textbf{Kendall's}} \\ \hline
\multicolumn{1}{|l|}{\textbf{Metrics}} & \multicolumn{1}{l|}{\textbf{$\rho$}} & \multicolumn{1}{l|}{\textbf{Z score}} & \textbf{P-value} & \multicolumn{1}{l|}{\textbf{$\tau$}} & \multicolumn{1}{l|}{\textbf{Z score}} & \textbf{P-value} \\ \hline
\multicolumn{1}{|l|}{LC vs BLEU} & \multicolumn{1}{l|}{0.0824} & \multicolumn{1}{l|}{0.2537} & 0.3999 & \multicolumn{1}{l|}{0.0769} & \multicolumn{1}{l|}{0.3674} & 0.3567 \\ \hline
\multicolumn{1}{|l|}{LC vs EM} & \multicolumn{1}{l|}{0.0769} & \multicolumn{1}{l|}{0.2367} & 0.4064 & \multicolumn{1}{l|}{0.0513} & \multicolumn{1}{l|}{0.2449} & 0.4032 \\ \hline
\multicolumn{1}{|l|}{LC vs CB} & \multicolumn{1}{l|}{0.0330} & \multicolumn{1}{l|}{0.1013} & 0.4597 & \multicolumn{1}{l|}{0.0256} & \multicolumn{1}{l|}{0.1225} & 0.4513 \\ \hline
\multicolumn{1}{|l|}{LC vs RL} & \multicolumn{1}{l|}{0.1703} & \multicolumn{1}{l|}{0.5283} & 0.2986 & \multicolumn{1}{l|}{0.1282} & \multicolumn{1}{l|}{0.6124} & 0.2701 \\ \hline
\multicolumn{1}{|l|}{LC vs MT} & \multicolumn{1}{l|}{0.1703} & \multicolumn{1}{l|}{0.5283} & 0.2986 & \multicolumn{1}{l|}{0.1282} & \multicolumn{1}{l|}{0.6124} & 0.2701 \\ \hline
\multicolumn{1}{|l|}{MS vs BLEU} & \multicolumn{1}{l|}{0.3352} & \multicolumn{1}{l|}{1.0708} & 0.1421 & \multicolumn{1}{l|}{0.2564} & \multicolumn{1}{l|}{1.2247} & 0.1103 \\ \hline
\multicolumn{1}{|l|}{MS vs EM} & \multicolumn{1}{l|}{0.3901} & \multicolumn{1}{l|}{1.2652} & 0.1029 & \multicolumn{1}{l|}{0.2564} & \multicolumn{1}{l|}{1.2247} & 0.1103 \\ \hline
\multicolumn{1}{|l|}{MS vs CB} & \multicolumn{1}{l|}{0.2967} & \multicolumn{1}{l|}{0.9396} & 0.1737 & \multicolumn{1}{l|}{0.2821} & \multicolumn{1}{l|}{1.3472} & 0.0890 \\ \hline
\multicolumn{1}{|l|}{MS vs RL} & \multicolumn{1}{l|}{0.4286} & \multicolumn{1}{l|}{1.4072} & 0.0797 & \multicolumn{1}{l|}{0.2821} & \multicolumn{1}{l|}{1.3472} & 0.0890 \\ \hline
\multicolumn{1}{|l|}{MS vs MT} & \multicolumn{1}{l|}{0.2967} & \multicolumn{1}{l|}{0.9396} & 0.1737 & \multicolumn{1}{l|}{0.2051} & \multicolumn{1}{l|}{0.9798} & 0.1636 \\ \hline
\end{tabular}}
\label{tab:rq3_toga}
\end{table}
